GooFit: A library for massively parallelising maximum-likelihood fits

Fitting complicated models to large datasets is a bottleneck of many analyses. We present GooFit, a library and tool for constructing arbitrarily-complex probability density functions (PDFs) to be evaluated on nVidia GPUs or on multicore CPUs using OpenMP. The massive parallelisation of dividing up event calculations between hundreds of processors can achieve speedups of factors 200-300 in real-world problems.

==> flow.tex <==
% This file no longer used. 
\section{Program flow and organisation}
\label{sec:flow}

This section should contain a diagram of the various GooFit modules,
plus the GPU and MINUIT (perhaps as literally black boxes). Also
an explanation in text of what the various things do. Then, a flow 
diagram of how the numbers pass back and forth during a fit. 


